Automatic Variational Inference in Stan

Variational inference is a scalable technique for approximate Bayesian inference. Deriving variational inference algorithms requires tedious model-specific calculations; this makes it difficult to automate. We propose an automatic variational inference algorithm, automatic differentiation variational inference (ADVI). The user only provides a Bayesian model and a dataset; nothing else. We make no conjugacy assumptions and support a broad class of models. The algorithm automatically determines an appropriate variational family and optimizes the variational objective. We implement ADVI in Stan (code available now), a probabilistic programming framework. We compare ADVI to MCMC sampling across hierarchical generalized linear models, nonconjugate matrix factorization, and a mixture model. We train the mixture model on a quarter million images. With ADVI we can use variational inference on any model we write in Stan.

==> img/normal_model_code.tex <==
\begin{lstlisting}
  data {
    int N;
    vector x[N]; // observations
  }

  parameters {
    // latent variable
    real mu;
  }

  model {
    // prior on latent variable
    mu ~ normal(0, 1.0);

    // likelihood
    for (n in 1:N)
      x[n] ~ normal(mu, 1.0);
  }
\end{lstlisting}

